Beam Search with Bidirectional Strategies for Neural Response Generation

Sequence-to-sequence neural networks have been widely used in language-based applications as they have flexible capabilities to learn various language models. However, when seeking for the optimal language response through trained neural networks, current existing approaches such as beam-search decoder strategies are still not able reaching to promising performances. Instead of developing various decoder strategies based on a "regular sentence order" neural network (a trained model by outputting sentences from left-to-right order), we leveraged "reverse" order as additional language model (a trained model by outputting sentences from right-to-left order) which can provide different perspectives for the path finding problems. In this paper, we propose bidirectional strategies in searching paths by combining two networks (left-to-right and right-to-left language models) making a bidirectional beam search possible. Besides, our solution allows us using any similarity measure in our sentence selection criterion. Our approaches demonstrate better performance compared to the unidirectional beam search strategy.

==> comments.tex <==
What is this paper about, and what contributions does it make?
> ---------------------------------------------------------------------------
> Problem/Question:
> Beam search is an essential technique for current RNN-based language
> generation models, in support of finding the most likely sequence,
> which typically achieves better performance than greedy search on
> various NLP tasks.
>
> Contributions
>         1. This work proposes two new beam search variants by utilizing an
> additional backward decoder. One is selecting sequences by
> interpolated scores between the forward and backward RNNs, and the
> other is by checking the agreement between two models on each
> hypothesis.
>         2. Both methods gain consistent improvement over the regular beam
> search. In experiments on QA and machine translation. The complexity
> analysis is helpful for determining its computational cost.
> ---------------------------------------------------------------------------
>
>
> What strengths does this paper have?
> ---------------------------------------------------------------------------
> Strengths (list at least two):
> 1. The motivation is clear and sensible. By incorporating a backward
> language model, it counteracts the long-term dependencies problem of
> unidirectional RNN.
> 2. The 2nd variant BidiA based on the Word Mover’s Distance works
> better and stabler. To some extent, it overcomes a common problem in
> traditional beam search: sequences ranked by likelihood don’t
> guarantee a better task-specific score, particularly under a large
> beam size, as shown in the Sec 3.2.
> ---------------------------------------------------------------------------
>
>
> What weaknesses does this paper have?
> ---------------------------------------------------------------------------
> Weaknesses (list at least two):
> 1. (-) The proposed algorithms rely on training an additional model (a
> backward language model), which results in higher training cost and a
> larger number of parameters.
> 2. (--) The performance improvement may result from the ensemble of
> two decoders more than from the improved beam search. More analysis
> and results are required to exclude such possibility.
> 3. (-) The scores of greedy search are not given, making us less
> certain about the necessity and benefit of using beam search.
> 4. (--) The BidiA presents good empirical results but its rationale is
> not clear to me. Determining the reason and looking for other
> surrogates of likelihood for beam search might be interesting topics
> for the future work.
> 5. Is the scale of BLEU in Figure 1 correct, about 1.60-1.68*10-4?
> 6. Overall, the topic is interesting and worth exploring. But the
> paper hasn’t given good answers to many problems it should address.
>
> Typos:
> P3 line 287, something is missing after “of”: We also observe that
> BidiA boosts the BLEU performance of by around 6%.
> P4 line 388, something is missing after “of the”: Poor performance of
> the is due to ...


What is this paper about, and what contributions does it make?
> ---------------------------------------------------------------------------
> Problem/Question:
> The paper presents a bidirectional beam search method for
> sequence-to-sequence tasks. They evaluate the method on a
> conversational dataset as well as the WMT14 English-Germany
> translation task. The results show improved performance over the
> corresponding baselines. In addition, several experimental analysis
> are conducted to demonstrate the advantages of the proposed method.
> One question is that why the BLEU scores of the English-Germany
> translation task are so pool.
>
>
> Contributions (list at least two):
> (1) propose an improved method for bidirectional beam search.
> (2) conduct several experiments to verify their method empirically.
> (3) theoretically demonstrate the effectiveness of the proposed method.
> ---------------------------------------------------------------------------
>
>
> What strengths does this paper have?
> ---------------------------------------------------------------------------
> Strengths (list at least two):
> (1) The proposed bidirectional decoding method BidiA is more balanced
> than the method BidiS, and meanwhile no additional hyper-parameter is
> required.
> (2) The method BidiA  is empirically significantly better than the
> baseline method as well as BidiS.
> (3) Experimental complexity and ranking analysis is interesting,
> showing the advantage of BidiA  in different viewpoints.
> ---------------------------------------------------------------------------
>
>
> What weaknesses does this paper have?
> ---------------------------------------------------------------------------
> Weaknesses (list at least two):
> (1) The BLEU scores of the English-Germany translation task are so
> pool. The authors would better check them.
> (2) Some important experimental results are not explained, for
> example, why BidiS performs poorly when beam size increases in Figure
> 1.
> (3) The importance of The Word Mover’s Distance should be verified in
> depth by comparisons.  I guess it is a key for BidiA.


What is this paper about, and what contributions does it make?
> ---------------------------------------------------------------------------
> Problem/Question:
> The paper identifies a shortcoming of standard beam-search decoder
> strategies, i.e. that they explore the output sequence from
> left-to-right. Instead, the paper proposes beam-search strategies that
> incorporate a "reverse" decoder as well.
>
> Contributions:
> - The paper proposes two bidirectional beam search strategies; both
> use a secondary decoder trained to generate the output sequences in
> reverse. The first strategy employs beam-search on the prime decoder,
> and reranks the outputs using a weighted average of the scores from
> the primary and reverse decoder. The second strategy generates
> sequences using both decoders and returns the sequence that minimizes
> the word mover's distance between itself and all other sequences.
> - The paper provides a complexity analysis of the proposed strategies
> that shows that the second proposed strategy is more efficient than
> standard beam-search.
> ---------------------------------------------------------------------------
>
>
> What strengths does this paper have?
> ---------------------------------------------------------------------------
> - The paper provides experimental results (across two different tasks)
> that show the proposed beam-search strategies consistently producing
> better sequences than the standard beam-search.
> - The paper theoretically shows that the second beam approach is more
> efficient than standard beam search, at least for beam of significant
> size.
> - The paper is clearly written, and the models should be easy to reproduce.
> ---------------------------------------------------------------------------
>
>
> What weaknesses does this paper have?
> ---------------------------------------------------------------------------
> - While the experiment results suggest consistent improvements when
> using the proposed strategies, the BLEU scores are very low overall.
> This implies that in the specific datasets the model output has very
> little overlap with the available references, which in turn makes it
> very hard to interpret the scores.
> - Given the unreliability of low BLEU scores, the paper could benefit
> from more output examples that clearly show how the reverse decoder
> helps improve the beam-search strategy.


> - The first proposed strategy is very similar to
> overgenerate-and-rerank methods used in generation, e.g. Wen et al.
> 2015 "Stochastic language generation in dialogue using recurrent
> neural networks with convolutional sentence reranking". Perhaps it
> could be framed as a sub-case of BidiS for a specific value of lambda.
> - Given the examples in Table 1, it's unclear to this reviewer how the
> proposed strategies improve on the output.



Here, we describe in depth the proposed method that integrate
forward and backward attentions. This approach is motivated
by the following two considerations.
First, attention-based encoder-decoder models are generally not good at decoding long utterances as mentioned in [9].
They tend to output less reliable labels in the latter part of utterances due to error accumulation. Figure 1 shows how many
substitution errors word-level forward and backward decoders
made at different relative positions of utterances in a Japanese
speech recognition experiment 1
. In this figure, the forward decoder made more errors than the backward counterpart in the
later part of utterances, while we observe an opposite tendency
in the earlier part. This shows that unidirectional decoders tend
to be more accurate at their early decoding steps, which leads
to a strategy that concatenates reliable parts of sequences obtained from two directional decoders. These newly generated
hypotheses can have fewer errors than the original ones, if this
concatenation process is managed in an appropriate way.
Second, because speech has an asymmetric time structure,
forward and backward decoders may have strengths in different ways which may contribute to better accuracy complementarily. Therefore, we expect a performance gain from simply
combining their recognition results, considering the consistent
effectiveness of the system combination approaches [18][19] in
many ASR tasks such as noisy speech recognition [20].

https://www.cs.cmu.edu/~sross1/publications/Ross-AIStats11-NoRegret.pdf \epsilon T**2



---------------------
In this section we compare the index returned by \textit{BidiA}, \textit{VBS} and \textit{Best Hypothesis} as shown in \autoref{}. We observe that for the \textit{Best Hypothesis} the distribution of return index is very similar for both corpus which is not the case for \textit{BidiA}. Although the very most likely sentences are not the one with the highest BLEU-4 we observe that a majority is ranked in the first half. For both dataset, we observe that $\textit{BidiA}_{BLEU}$ distribution is more simi

A faire :

Selon la likelihood + ajouter best hypothesis
Rank analysis: 
best hypothesis selon la likelhood et celle du bleu score 
corpus dependant
not all with 20 
remonter en 3.3
Index dans la beam selon la likelihood



------
Faire un toru sur les refs




